An AI-Native Runtime for Multi-Wearable Environments

The miniaturization of AI accelerators is paving the way for next-generation wearable applications within wearable technologies. We introduce Mojito, an AI-native runtime with advanced MLOps designed to facilitate the development and deployment of these applications on wearable devices. It emphasizes the necessity of dynamic orchestration of distributed resources equipped with ultra-low-power AI accelerators to overcome challenges associated with unpredictable runtime environments. Through its innovative approaches, Mojito demonstrates how future wearable technologies can evolve to be more autonomous.

==> sections/proteus.tex <==
\section{TIME-BOUND CONTEXTUAL BIO-ID}

We introduce an innovative concept: \emph{time-bound contextual bio-IDs}, to provide instant and efficient device-to-device authentication~\cite{proteus}. These are universal representations of sensor data embedded in a common latent space, ensuring individuality across different users and contexts. More specifically, we extract a time-bound bio-ID from vital signs such as heart rate, oxygen saturation, and blood pressure. These metrics are inherently universal for an individual regardless of the device placement, but unique according to the individual’s dynamic and contextual factors. For instance, the system, like a smartphone, can detect shared use and activate privacy-enhanced mode for secure communication on smart earbuds by comparing bio-IDs generated from each earbud.

To generate the bio-IDs we leverage contrastive learning to extract the common latent space of vital sign signals: positive pairs consist of sensor data coming from multiple wearables worn by the same user at the same time, while data from different users or different time points act as negative pairs, pushing for disparate embeddings. Our evaluation with several multi-modal datasets across multiple device placements, users, and activities shows that we can process these embeddings with a high quality such that even when the raw data does not show any correlation the resulting embeddings are aligned when the devices are on the same body at the same time. Figure~\ref{fig:results} (b) shows an example of a PPG signal and the corresponding embeddings on two earbuds for the same user and different users. The results show that our bio-IDs are also time-bound, which means that the embeddings are different even from the same user when they are generated at different times. 



==> sections/thermal.tex <==
\section{THERMAL COMFORT MANAGEMENT}

Thermal management in wearable environments is crucial for maintaining user comfort and device performance. A common approach to thermal regulation is Dynamic Voltage and Frequency Scaling (DVFS), which adjusts the voltage and frequency of a processor based on the workload demand. This method reduces the power consumption and consequently the heat generation, thus managing the device's temperature. However, it brings unavoidable performance degradation. Passive cooling techniques, like heat sinks or thermal conduction materials, are also used to distribute or dissipate heat without using power, but it is not yet widely adopted in today's wearables due to the size limit and cost. Most importantly, they address the thermal problem mostly from the resource perspective, so they mostly lack the view of thermal comfort management.

In \system{}, we develop a novel approach for thermal comfort management for wearable devices. It considers both device wearability and user-perceived heat, leveraging the multiplicity of devices. More specifically, it employs three key innovative techniques. First, it performs profiling and modeling of the relationship between device workload and actual temperature measured at the position where the user's skin is attached. Second, by using various sensors like IMU and proximity sensors, it predicts the wear status of each device, i.e., whether the device is on the body or on the desk. Then, it distributes tasks across multiple devices in a way to avoid a situation where the predicted skin-contact temperature is higher than the threshold, considering skin temperature and wearability. For example, if one device is placed on the desk, higher heat from processing more tasks would be acceptable as it does not directly harm the user's skin at the moment.


% we propose a novel heat orchestration method for wearable devices, leveraging the unique characteristics of on-body proactive AI applications, i.e., the multiplicity of devices. More specifically, instead of 

% It employs predictive algorithms to anticipate thermal outputs based on various operational parameters, ensuring that the heat generated by the devices remains within safe limits for user contexts.
